The Lagrangian Numerical Relativity code SPHINCS_BSSN_v1.0

We present version 1.0 of our Lagrangian Numerical Relativity code SPHINCS_BSSN. This code evolves the full set of Einstein equations, but contrary to other Numerical Relativity codes, it evolves the matter fluid via Lagrangian particles in the framework of a high-accuracy version of Smooth Particle Hydrodynamics (SPH). The major new elements introduced here are: i) a new method to map the stress--energy tensor (known at the particles) to the spacetime mesh, based on a local regression estimate; ii) additional measures that ensure the robust evolution of a neutron star through its collapse to a black hole; and iii) further refinements in how we place the SPH particles for our initial data. The latter are implemented in our code SPHINCS_ID which now, in addition to LORENE, can also couple to initial data produced by the initial data library FUKA. We discuss several simulations of neutron star mergers performed with SPHINCS_BSSN_v1.0, including irrotational cases with and without prompt collapse and a system where only one of the stars has a large spin ($\chi = 0.5)$.

==> own_latex_commands_i.tex <==
% own commands
\newcommand{\nifs}{\ensuremath{^{56}\mathrm{Ni}}}
\newcommand{\Nifs}{\ensuremath{^{56}\mathrm{Ni}} $\;$}
\def\paren#1{\left( #1 \right)}
\def\Mesz{M\'esz\'aros~}
\def\Pacz{Paczy\'nski~}
\def\Kluz{Klu\'zniak~}
\def\p{\partial}
\def\msun{M$_{\odot}$}
\def\Msun{M$_{\odot}$ }
\def\be{\begin{equation}}
\def\ee{\end{equation}}
\def\bi{\begin{itemize}}
\def\i{\item}
\def\ei{\end{itemize}}
\def\ben{\begin{enumerate}}
\def\een{\end{enumerate}}
\def\bea{\begin{eqnarray}}
\def\eea{\end{eqnarray}}
\def\bt{\begin{tabbing}}
\def\et{\end{tabbing}}
\def\gcc{gcm$^{-3}$}
\def\Gcc{gcm$^{-3} \;$}
\def\ccm{cm$^3$}
\def\edo{\end{document}}
\def\red{\textcolor{red}}
\def\blue{\textcolor{blue}}
\def\green{\textcolor{green}}
\def\ye{$Y_e$}
\def\Ye{$Y_e$ }
\def\rs{$R_{\rm S}$}
\def\Rs{$R_{\rm S}$ }
\def\noin{\noindent}
\def\QIone{\mathcal{Q}_{\; \; 1}}
\def\QItwo{\mathcal{Q}_{\; \; 2}}
\def\QIthree{\mathcal{Q}_{\; \; 3}}
\def\QIfour{\mathcal{Q}_{\; \; 4}}
\newcommand{\ud}{\mathrm{d}}
\newcommand{\sn}{\ensuremath{\mathrm{sn}}}
\newcommand{\cn}{\ensuremath{\mathrm{cn}}}
\newcommand{\dn}{\ensuremath{\mathrm{dn}}}
\newcommand{\sech}{\ensuremath{\mathrm{sech}}}
\newcommand{\nd}{\noindent}
\newcommand{\enth}{\mathcal{E}}
\newcommand{\carb}{$^{12}$C}
\newcommand{\Carb}{$^{12}$C $\;$}
\newcommand{\ox}{$^{16}$O}
\newcommand{\Ox}{$^{16}$O $\;$}
\newcommand{\tlg}{\tilde{\gamma}}
\newcommand{\tlG}{\tilde{\Gamma}}
\newcommand{\emfp}{e^{-4\phi}}
\newcommand{\tlA}{\tilde{A}}
\newcommand{\tlR}{\tilde{R}}
\newcommand{\xt}{\tilde{x}}
\newcommand{\dt}[1]{\partial_t #1}
\newcommand{\pdu}[3]{\partial_{#3} #1^{#2}}
\newcommand{\pdl}[3]{\partial_{#3} #1_{#2}}
\newcommand{\pdpdu}[4]{\partial_{#3}\partial_{#4} #1^{#2}}
\newcommand{\pdpdl}[4]{\partial_{#3}\partial_{#4} #1_{#2}}
\newcommand{\upwindu}[3]{\beta^{#3}\bar{\partial}_{#3} #1^{#2}}
\newcommand{\upwindl}[3]{\beta^{#3}\bar{\partial}_{#3} #1_{#2}}
%\newcommand{\comment}[1]{{\color{red}$\blacksquare$~\textsf{[#1]}}}
\newcommand{\tlGn}{\tilde{\Gamma}_{\mathrm{(n)}}}
\newcommand{\tlGmixed}[2]{\tlG_{#1}^{\;\;\;#2}}



% Oleg's special
\def\peak{\rm peak}
\def\ji{\varphi}
\def\rin{\mathcal{I}}
\def\x{{\bf x}}
\def\s{{\bf s}}
\def\k{{\bf k}}
\def\n{{\bf n}}
\def\f{{\bf f}}
\def\pd{\partial}
\def\fa{f_{\alpha}(\x,\p,t)}
\def\kabs{\kappa^{\rm abs}_\nu}
\def\ksca{\kappa^{\rm sca}_\nu}
\def\Flux{{\bf F}_\nu}
\def\Frad{{\bf F}_{\rm rad}}
\def\Pressure{{\mathsf P}_\nu}
\def\kB{k_B}
\def\tauph{\tau_{\it ph}}
\def\taumu{\tau_\mu}
\def\MSun{M_{\astrosun}}


% Journals
\newcommand{\apj}{Ap. J., }
\newcommand{\apjl}{Ap. J. Lett., }
\newcommand{\apjs}{Ap. J. Supp., }
\newcommand{\physrep}{Phys. Rep., }
\newcommand{\mnras}{Mon. not. RAS., }
\newcommand{\apss}{Astroph. \& Space Sci., }
\newcommand{\aap}{Astron. \& Astrophys., }
\newcommand{\prc}{Phys. Rev. C.,} 
\newcommand{\prd}{Phys. Rev. D.,} 
\newcommand{\nat}{Nature,}
\newcommand{\pasp}{Publications of the Astronomical Society of the Pacific,}

% SPH kernels
\def\M4{M$_4$}
\def\M6{M$_6$}
\def\lcm6{LCM$_6$}
\def\qcm6{QCM$_6$}
\def\whn{W$_{\rm H,n}$}
\def\wh3{W$_{\rm H,3}$}
\def\wh4{W$_{\rm H,4}$}
\def\wh5{W$_{\rm H,5}$}
\def\wh6{W$_{\rm H,6}$}
\def\wh7{W$_{\rm H,7}$}

% vector algebra
\def\divv{\nabla \cdot \vec{v}}
\def\vv{\vec{v}}
\def\dx{\Delta x}

% alternative vector symbole
\newcommand{\ve}[1]{\boldsymbol{#1}}

% turbulence
\def\ed{\dot{\epsilon}}
\def\vl{v_\lambda}
\def\vort{\vec{\mathcal{W}}}

% reduced quadrupole moment
\newcommand{\rqm}{{%
      \declareslashed{}{\text{-}}{0.04}{0}{I}\slashed{I}}}

% code names
\newcommand{\SpB}{\texttt{SPHINCS\_BSSN}\; }
\newcommand{\spB}{\texttt{SPHINCS\_BSSN}}
\newcommand{\spB1}{\texttt{SPHINCS\_BSSN}\_v1.0}
\newcommand{\spid}{\texttt{SPHINCS\_ID}}
\newcommand{\spiD}{\texttt{SPHINCS\_ID}\; }
\newcommand{\Ma}{\texttt{MAGMA2}\;}
\newcommand{\ma}{\texttt{MAGMA2}}
\newcommand{\Lo}{\texttt{LORENE}\;}
\newcommand{\lo}{\texttt{LORENE}}
\newcommand{\Fu}{\texttt{FUKA}\;}
\newcommand{\fu}{\texttt{FUKA}}
\newcommand{\comp}{\texttt{CompOSE}\;}
\newcommand{\binns}{\texttt{BinNS}\;}
\newcommand{\McL}{\texttt{McLachlan}\;}
\newcommand{\Mhdu}{\texttt{MHDUET}\;}
\newcommand{\mhdu}{\texttt{MHDUET}}
\newcommand{\Sam}{\texttt{SAMRAI}\;}
\newcommand{\sam}{\texttt{SAMRAI}}
\newcommand{\Simf}{\texttt{Simflowny}\;}
\newcommand{\simf}{\texttt{Simflowny}}







